Post-hoc Self-explanation of CNNs

Although standard Convolutional Neural Networks (CNNs) can be mathematically reinterpreted as Self-Explainable Models (SEMs), their built-in prototypes do not on their own accurately represent the data. Replacing the final linear layer with a $k$-means-based classifier addresses this limitation without compromising performance. This work introduces a common formalization of $k$-means-based post-hoc explanations for the classifier, the encoder's final output (B4), and combinations of intermediate feature activations. The latter approach leverages the spatial consistency of convolutional receptive fields to generate concept-based explanation maps, which are supported by gradient-free feature attribution maps. Empirical evaluation with a ResNet34 shows that using shallower, less compressed feature activations, such as those from the last three blocks (B234), results in a trade-off between semantic fidelity and a slight reduction in predictive performance.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}





% our stuff starts here
\usepackage{microtype} % helps \looseness=-1 a lot, I hope this is legal :D

\usepackage{tabularx}
\usepackage{color}
\usepackage{amsmath,amssymb,amstext,amsfonts,amsthm}
\usepackage{multirow}
\usepackage{bbm}
\usepackage{bm}
% \usepackage{wrapfig}

\RequirePackage{booktabs}

\usepackage{mathtools}

\renewcommand{\tabcolsep}{2pt}

\usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{algpseudocode}
%\usepackage{bibtopic}


% use ttfamily for algorithm
\makeatletter
\algrenewcommand\ALG@beginalgorithmic{\ttfamily}
\makeatother


% \newcommand{\comment}[1]{\textbf{\textcolor{blue}{#1}}}
% \newcommand{\todo}[1]{\textbf{\textcolor{red}{#1}}}

\newcommand{\edit}[1]{{\textcolor{red}{#1}}}
\newcommand{\editnew}[1]{{\textcolor{blue}{#1}}}

\newcommand{\isep}{\mathrel{{.}\,{.}}\nobreak}
\newcommand{\rsep}{\, ,\nobreak}

\newcommand{\balpha}{{\bm \alpha}}

\newcommand{\B}{{\bm B}}

\newcommand{\bc}{{\bm c}}
\newcommand{\tc}{\tilde{\bc}}

\newcommand{\bI}{\mathbf{I}}

\newcommand{\cL}{\mathcal{L}}
\newcommand{\cl}{\ell}

%\DeclareMathOperator*{\E}{\mathbbm{E}}

\newcommand{\bGamma}{{\bm \Gamma}}

\newcommand{\I}{{\bm I}}

\newcommand{\bmu}{{\bm \mu}}

\DeclareMathOperator*{\N}{\mathbbm{N}}

\newcommand{\bphi}{{\bm \phi}}
\newcommand{\bPhi}{{\bm \Phi}}

\newcommand{\cQ}{\mathcal{Q}}

%\DeclareMathOperator*{\R}{\mathbbm{R}}
\newcommand{\Rp}{{\R}_{\geq0}}


\newcommand{\s}{{\bm s}}
\newcommand{\bsigma}{{\bm \sigma}}

\newcommand{\X}{{\bm X}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\x}{{\bm x}}
\newcommand{\hx}{\hat{\x}}
\newcommand{\tx}{\bar{\x}}
\newcommand{\tX}{\bar{\X}}

\newcommand{\y}{{\bm y}}
\newcommand{\hy}{\hat{\y}}
\newcommand{\cY}{\mathcal{Y}}

\newcommand{\z}{{\bm z}}
\newcommand{\tz}{\tilde{\bz}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}

\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{#1\;\delimsize\|\;#2}
\newcommand{\dkl}{\mathrm{D}_\mathrm{KL}\infdivx}

%\newcommand{\argmax}{\operatorname{argmax}}
\usepackage{enumitem}

%\usepackage{graphicx}
%\usepackage{siunitx}
%\DeclareMathAlphabet{\mymathbb}{U}{BOONDOX-ds}{m}{n}
%\graphicspath{{img/}}
%\newtheorem{definition}{Definition}
\usepackage{multirow}
%\clubpenalty10000
%\widowpenalty10000


\newcommand{\avgpool}{\operatorname{avg.pool}}
\newcommand{\enc}{\operatorname{enc}}
\newcommand{\clf}{\operatorname{clf}}
\newcommand{\simm}{\operatorname{sim}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\att}{\operatorname{att}}
\usepackage{mathtools}


\newtheorem{theorem}{Theorem}


\DeclareFontFamily{U}{mathx}{}
\DeclareFontShape{U}{mathx}{m}{n}{<-> mathx10}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareMathAccent{\widehat}{0}{mathx}{"70}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}
